Back to the Drawing Board for Fair Representation Learning

The goal of Fair Representation Learning (FRL) is to mitigate biases in machine learning models by learning data representations that enable high accuracy on downstream tasks while minimizing discrimination based on sensitive attributes. The evaluation of FRL methods in many recent works primarily focuses on the tradeoff between downstream fairness and accuracy with respect to a single task that was used to approximate the utility of representations during training (proxy task). This incentivizes retaining only features relevant to the proxy task while discarding all other information. In extreme cases, this can cause the learned representations to collapse to a trivial, binary value, rendering them unusable in transfer settings. In this work, we argue that this approach is fundamentally mismatched with the original motivation of FRL, which arises from settings with many downstream tasks unknown at training time (transfer tasks). To remedy this, we propose to refocus the evaluation protocol of FRL methods primarily around the performance on transfer tasks. A key challenge when conducting such an evaluation is the lack of adequate benchmarks. We address this by formulating four criteria that a suitable evaluation procedure should fulfill. Based on these, we propose TransFair, a benchmark that satisfies these criteria, consisting of novel variations of popular FRL datasets with carefully calibrated transfer tasks. In this setting, we reevaluate state-of-the-art FRL methods, observing that they often overfit to the proxy task, which causes them to underperform on certain transfer tasks. We further highlight the importance of task-agnostic learning signals for FRL methods, as they can lead to more transferrable representations.

==> Makefile <==
# Makefile, allowing to
# - compile
# - test
# - clean
# - run in docker
# For details, see targets defined below
#
# USAGE, for example: make pdf

#####################
# REQUIRED PACKAGES #
#####################

# For instructions on how to set up your system to run all commands here, follow
# https://hub.docker.com/repository/docker/ethsrilab/latex-plus

##############
# PARAMETERS #
##############

# main
OUTPUTDIR := lqa-output
NAME := main

# special
NOAPPENDIX := $(NAME)_no_appendix
FULL := $(NAME)_full
OVERFULL := $(NAME)_overfull
GRAY := $(NAME)_gray
ABSTRACT := $(OUTPUTDIR)/abstract.txt

# submission
SUBMISSIONDIR := submission
ZIP := submission.zip

# log
LATEXMKDIR := $(OUTPUTDIR)/latexmk
LOG := $(OUTPUTDIR)/$(NAME).log
SHORTLOG := $(OUTPUTDIR)/$(NAME)-short.log

LOGFILES := *.aux *.bbl *.log *.bcf  *.blg *.lot *.toc *.swp *.gz *.out *.ttt *.fls *.fdb_latexmk

# scripts

SCRIPTDIR := lqa/scripts

#############
# COMPILING #
#############

LATEXSCRIPT = ./lqa/latex.sh
LATEX := $(LATEXSCRIPT) $(NAME).tex $(LATEXMKDIR)

##########
# OTHERS #
##########

NOAPPENDIXCONFIG := headers/config/noappendix.config
SHOWOVERFULLCONFIG := headers/config/showoverfull.config

########
# PDFS #
########

.DEFAULT_GOAL := pdf-full

.PHONY: pdf-full
pdf-full:
	# cleanminimal required to remove the root .bbl file (latexmk is confused by this)
	make cleanminimal
	@echo "\n> COMPILING pdf..."
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(FULL).pdf
	@cp $(LATEXMKDIR)/$(NAME).bbl $(OUTPUTDIR) || true
	@cp $(LATEXMKDIR)/$(NAME).log $(LOG)

.PHONY: pdf-appendix
pdf-appendix: pdf-full
	python3 $(SCRIPTDIR)/pages.py --action appendix

# generate labels into the appendix
.PHONY: appendix-labels
appendix-labels: pdf-full
	cat lqa/other/appendix-labels-loader-1.tex > appendix-labels-loader.tex
	# On error "cat: lqa-output/latexmk/appendix.aux: No such file or directory" check if \include{appendix} is still in main.tex 
	cat $(LATEXMKDIR)/appendix.aux >> appendix-labels-loader.tex
	cat lqa/other/appendix-labels-loader-2.tex >> appendix-labels-loader.tex

# generate PDF without the appendix, but with correct labels into the appendix
.PHONY: pdf-no-appendix
pdf-no-appendix: appendix-labels
	# force re-build of latexmk due to missing file
	make clean
	touch $(NOAPPENDIXCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(NOAPPENDIX).pdf
	# cleanminimal is not sufficient as latexmk will not rebuild during next iteration
	make clean

.PHONY: pdf-overfull
pdf-overfull:
	@echo "\n> COMPILING OVERFULL pdf..."
	# force re-build of latexmk due to missing file
	make clean
	touch $(SHOWOVERFULLCONFIG)
	$(LATEX)
	@cp $(LATEXMKDIR)/$(NAME).pdf $(OUTPUTDIR)/$(OVERFULL).pdf
	# cleanminimal is not sufficient as latexmk will not rebuild during next iteration
	make clean

.PHONY: pdf-gray
pdf-gray: pdf-full
	@echo "\n> Producing GRAYSCALE version to $(OUTPUTDIR)/$(GRAY).pdf..."
	gs -sOutputFile=$(OUTPUTDIR)/$(GRAY).pdf -sDEVICE=pdfwrite -sColorConversionStrategy=Gray -dProcessColorModel=/DeviceGray -dCompatibilityLevel=1.4 -qQUIET -dNOPAUSE -dBATCH $(OUTPUTDIR)/$(FULL).pdf

.PHONY: pdf-all
pdf-all: cleanall
	make pdf-appendix
	make pdf-no-appendix
	make pdf-overfull
	make pdf-gray
	make pdf-full

# build full pdf but also create synctex files
.PHONY: pdf-full-sync
pdf-full-sync: LATEX += "-synctex=1"
pdf-full-sync: pdf-full
	@cp $(LATEXMKDIR)/$(NAME).synctex.gz $(OUTPUTDIR)/$(FULL).synctex.gz || true


# produce better log files
.PHONY: log
log: pdf-full
	pplatex -i $(LOG) > $(SHORTLOG)


###############
# CONVENIENCE #
###############

.PHONY: check
check: pdf-full log
	python3 $(SCRIPTDIR)/checks.py

.PHONY: text
text: pdf-full
	pdftotext $(OUTPUTDIR)/$(FULL).pdf -raw $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/-\n//g' $(OUTPUTDIR)/$(FULL).txt
	sed -z -i 's/\n/ /g' $(OUTPUTDIR)/$(FULL).txt

.PHONY: all
all:
	make pdf-all
	make check
	make log

#########
# CLEAN #
#########

# make clean: remove temporary files
.PHONY: clean
clean:
	make cleanminimal
	@echo "\n> CLEANING temporary files..."
	rm -r -f $(LATEXMKDIR) || true
	rm -r -f $(OUTPUTDIR)/script-logs/*.log* || true
	cd $(OUTPUTDIR) && rm -f $(LOGFILES) || true

# make cleanall: remove all produced files
.PHONY: cleanall
cleanall:
	make clean
	@echo "\n> CLEANING PDFs..."
	rm -f *.pdf || true
	rm -f $(OUTPUTDIR)/*.pdf || true
	rm -r -f $(SUBMISSIONDIR) || true
	rm -f appendix-labels-loader.tex
	rm -f $(ABSTRACT)

# make cleanminimal: remove only temporary files in root directory
# - this removes the root .bbl file (latexmk is confused by this)
# - this removes temporary config files (required for appendix loader and overfull)
.PHONY: cleanminimal
cleanminimal:
	@echo "\n> CLEANING minimal files..."
	rm -f $(LOGFILES) || true
	rm -f headers/config/*.config

##############
# SUBMISSION #
##############

.PHONY: abstract
abstract:
	python3 $(SCRIPTDIR)/abstract.py

.PHONY: submission-files
submission-files:
	make cleanall
	make abstract
	# pdf-full omitted as pdf-appendix implicitly runs this
	make pdf-appendix
	make pdf-no-appendix

.PHONY: submission
submission: submission-files check
	@echo "\n> PREPARING submission in directory $(SUBMISSIONDIR)..."
	rm -r -f $(SUBMISSIONDIR)
	mkdir $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.pdf $(SUBMISSIONDIR)
	cp $(ABSTRACT) $(SUBMISSIONDIR)
	cp $(OUTPUTDIR)/*.bbl $(SUBMISSIONDIR)

.PHONY: zip-no-appendix
zip-no-appendix: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-no-appendix # update output, prepare appendix labels
	touch $(NOAPPENDIXCONFIG) # ensure appendix is not included when compiling again
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip Makefile
	make cleanminimal

.PHONY: zip-full
zip-full: submission
	@rm -f $(SUBMISSIONDIR)/$(ZIP)
	make pdf-full # update output
	# README_publisher.md is wrong in this case
	zip --quiet -r $(SUBMISSIONDIR)/$(ZIP) . -x /.git* /$(OUTPUTDIR)* /$(SUBMISSIONDIR)/*.zip Makefile README_publisher.md


#########
# ARXIV #
#########

.PHONY: arxiv-files
arxiv-files:
	make clean
	# clean up outdated directories
	rm -rf arxiv ._arXiv

	# create clean directory
	arxiv_latex_cleaner .
	# rename directory
	mv ._arXiv arxiv

	# copy bbl file
	make pdf-full
	cp $(OUTPUTDIR)/*.bbl ./arxiv

	# cleanup
	rm -f arxiv/Makefile arxiv/README.md arxiv/README_publisher.md

.PHONY: arxiv-check
arxiv-check: pdf-full arxiv-files
	# create pdf
	cd arxiv && latexmk -pdf -interaction=nonstopmode $(NAME).tex

	# check resulting pdf
	# requires pdfdiff: https://github.com/cascremers/pdfdiff
	echo "Differences between two PDFs:"
	pdfdiff --diffviewer diff $(OUTPUTDIR)/$(FULL).pdf ./arxiv/$(NAME).pdf

.PHONY: arxiv
arxiv: arxiv-files
	zip -r $(OUTPUTDIR)/arxiv.zip arxiv

##########
# DOCKER #
##########

DOCKER-CMD := ./lqa/docker.sh


PAPERDIR := $$(pwd)
IMAGE := ethsrilab/latex-plus:version-4.0
CONTAINER := latex-plus-container
RUN := $(DOCKER-CMD) run \
		-it \
		--name $(CONTAINER) \
		--workdir="/paper" \
		-v "$(PAPERDIR)":/paper \
		$(IMAGE)

# launch a docker container using the image, which will provide a shell in the container
.PHONY: docker-run
docker-run: clean-container
	$(RUN)

# check for updates and remove the created docker container
.PHONY: clean-container
clean-container:
	$(DOCKER-CMD) pull $(IMAGE)
	$(DOCKER-CMD) rm /$(CONTAINER) 2>/dev/null || true

# all above commands, run in docker
.PHONY: docker-all
docker-all: clean-container
	$(RUN) make all

.PHONY: docker-pdf-full
docker-pdf-full: clean-container
	$(RUN) make pdf-full

.PHONY: docker-pdf-full-sync
docker-pdf-full-sync: clean-container
	$(RUN) make pdf-full-sync

.PHONY: docker-pdf-appendix
docker-pdf-appendix: clean-container
	$(RUN) make pdf-appendix

.PHONY: docker-pdf-no-appendix
docker-pdf-no-appendix: clean-container
	$(RUN) make pdf-no-appendix

.PHONY: docker-pdf-overfull
docker-pdf-overfull: clean-container
	$(RUN) make pdf-overfull

.PHONY: docker-pdf-gray
docker-pdf-gray: clean-container
	$(RUN) make pdf-gray

.PHONY: docker-pdf-all
docker-pdf-all: clean-container
	$(RUN) make pdf-all

.PHONY: docker-submission
docker-submission: clean-container
	$(RUN) make submission

.PHONY: docker-check
docker-check: clean-container
	$(RUN) make check

.PHONY: docker-text
docker-text: clean-container
	$(RUN) make text

.PHONY: docker-zip
docker-zip: clean-container
	$(RUN) make zip

.PHONY: docker-zip-no-appendix
docker-zip-no-appendix: clean-container
	$(RUN) make zip-no-appendix

.PHONY: docker-abstract
docker-abstract: clean-container
	$(RUN) make abstract

.PHONY: docker-arxiv
docker-arxiv: clean-container
	$(RUN) make arxiv

.PHONY: docker-arxiv-check
docker-arxiv-check: clean-container
	$(RUN) make arxiv-check

